Synthesis of safety certificates for discrete-time uncertain systems via convex optimization

We study the problem of co-designing control barrier functions and linear state feedback controllers for discrete-time linear systems affected by additive disturbances. For disturbances of bounded magnitude, we provide a semi-definite program whose feasibility implies the existence of a control law and a certificate ensuring safety in the infinite horizon with respect to the worst-case disturbance realization in the uncertainty set. For disturbances with unbounded support, we rely on martingale theory to derive a second semi-definite program whose feasibility provides probabilistic safety guarantees holding joint-in-time over a finite time horizon. We examine several extensions, including (i) encoding of different types of input constraints, (ii) robustification against distributional ambiguity around the true distribution, (iii) design of safety filters, and (iv) extension to general safety specifications such as obstacle avoidance.

==> commands.tex <==
%============== General ================%
\newcommand{\reals}{\mathbb{R}}
\newcommand{\nonnegativeReals}{\mathbb{R}_{\geq 0}}
\newcommand{\positiveReals}{\mathbb{R}_{>0}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\Id}{\mathrm{Id}}
\renewcommand{\d}{\mathrm{d}}
\DeclareMathOperator*{\range}{Range}
\DeclareMathOperator*{\kernel}{Ker}
\newcommand{\ones}{\mathbbm{1}}
\newcommand{\zeros}{\mathds{O}}
\newcommand{\eye}{I}
\newcommand{\transpose}[1]{#1^\top}
\newcommand{\T}[1]{\transpose{#1}}
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\inv}[1]{\inverse{#1}}
\newcommand{\pseudoinverse}[1]{#1^\dagger}
\newcommand{\pinv}[1]{\pseudoinverse{#1}}
\newcommand{\sample}[2]{#1^{(#2)}}
\newcommand{\entry}[2]{#1_{#2}}

%============== Probabilities ================%
\newcommand{\Q}{\mathbb{Q}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\empiricalP}[1]{\widehat\P_{#1}}
\newcommand{\empiricalQ}[1]{\widehat\Q_{#1}}
\newcommand{\expectedValue}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\lebesgueMeasure}[1]{\mathcal{L}^{#1}}
\newcommand{\diracDelta}[1]{\delta_{#1}}
\newcommand{\support}[1]{\text{supp}(#1)}

%============== Functions ================%
\newcommand{\tensorProd}[2]{#1\times #2}
\newcommand{\proj}[1]{\pi_{#1}}
\newcommand{\indicator}[1]{\ones_{#1}}

%============== OT-related commands ================%
\newcommand{\setPlans}[2]{\Pi(#1,#2)}
\newcommand{\probSpace}[1]{\mathcal{P}(#1)}
\newcommand{\Pp}[2]{\mathcal{P}_{#1}(#2)}
\newcommand{\pushforward}[1]{{#1}_{\#}}
\newcommand{\transportCost}[3]{W^{#1}(#2,#3)}
\newcommand{\kl}[2]{\text{KL}(#1\Vert #2)}
\newcommand{\tv}[2]{\text{TV}(#1,#2)}
\newcommand{\ball}[3]{\mathbb{B}_{#1}^{#2}(#3)}

%============== Math operators ================%
\let\argmin\relax
\let\argmax\relax
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\epi}{epi}
\DeclareMathOperator*{\lip}{lip}

%============== Comments ================%
\newcommand\margincomment[4]{{\color{#3}#1}\marginpar{\vspace{-0\baselineskip}\color{#3}\raggedright\scriptsize [#4]:#2}}
\newcommand{\nlmargin}[2]{\margincomment{#1}{#2}{red}{NL}}
\newcommand{\lamargin}[2]{\margincomment{#1}{#2}{blue}{LA}}

==> graphics/safety.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1.2,xscale=1.2]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp0044176096267762865] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (102,69.43) -- (215.43,69.43) -- (215.43,171.43) -- (102,171.43) -- cycle ;
%Shape: Polygon [id:ds5309575007412408] 
\draw  [fill={rgb, 255:red, 228; green, 239; blue, 214 }  ,fill opacity=1 ] (151.43,75.43) -- (210.43,106.43) -- (171.43,163.43) -- (119.43,155.43) -- (111,106) -- cycle ;
%Shape: Circle [id:dp15887306560754744] 
\draw  [fill={rgb, 255:red, 240; green, 225; blue, 254 }  ,fill opacity=1 ] (124.43,135.93) .. controls (124.43,126.26) and (132.26,118.43) .. (141.93,118.43) .. controls (151.59,118.43) and (159.43,126.26) .. (159.43,135.93) .. controls (159.43,145.59) and (151.59,153.43) .. (141.93,153.43) .. controls (132.26,153.43) and (124.43,145.59) .. (124.43,135.93) -- cycle ;
%Shape: Rectangle [id:dp1739234572106254] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (227,69.43) -- (340.43,69.43) -- (340.43,171.43) -- (227,171.43) -- cycle ;
%Shape: Polygon [id:ds9151513799127085] 
\draw  [fill={rgb, 255:red, 228; green, 239; blue, 214 }  ,fill opacity=1 ] (276.43,75.43) -- (335.43,106.43) -- (296.43,163.43) -- (244.43,155.43) -- (236,106) -- cycle ;
%Shape: Circle [id:dp38910062860868155] 
\draw  [fill={rgb, 255:red, 240; green, 225; blue, 254 }  ,fill opacity=1 ] (249.43,135.93) .. controls (249.43,126.26) and (257.26,118.43) .. (266.93,118.43) .. controls (276.59,118.43) and (284.43,126.26) .. (284.43,135.93) .. controls (284.43,145.59) and (276.59,153.43) .. (266.93,153.43) .. controls (257.26,153.43) and (249.43,145.59) .. (249.43,135.93) -- cycle ;
%Shape: Free Drawing [id:dp939596249346776] 
\draw  [line width=0.75] [line join = round][line cap = round] (131.43,138.43) .. controls (120.91,138.43) and (121.12,135.51) .. (118.43,127.43) .. controls (117.76,125.43) and (115.92,123.47) .. (116.43,121.43) .. controls (118.17,114.46) and (127.9,114.96) .. (132.43,110.43) .. controls (135.78,107.07) and (134.04,102.21) .. (136.43,97.43) .. controls (138.79,92.71) and (149.21,93.11) .. (152.43,93.43) .. controls (153.3,93.52) and (154.8,95.6) .. (155.43,96.43) .. controls (157.03,98.57) and (160.58,103.13) .. (159.43,105.43) .. controls (158.1,108.09) and (153.2,108.86) .. (155.43,114.43) .. controls (156.43,116.94) and (165.66,114.96) .. (162.43,121.43) .. controls (161.59,123.11) and (155.11,123.38) .. (154.43,125.43) .. controls (150.16,138.24) and (155.98,138.12) .. (166.43,139.43) .. controls (167.79,139.6) and (169.12,140.86) .. (170.43,140.43) .. controls (175.37,138.78) and (184.34,122.08) .. (183.43,118.43) .. controls (182.91,116.37) and (176.73,113.95) .. (176.43,112.43) .. controls (175.28,106.7) and (185.68,100.68) .. (179.43,94.43) .. controls (174.22,89.22) and (168.43,92.95) .. (168.43,98.43) ;
%Shape: Free Drawing [id:dp07810501371612388] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75] [line join = round][line cap = round] (256.43,136.43) .. controls (247.08,136.43) and (245.67,120.97) .. (246.43,113.43) .. controls (246.66,111.14) and (254.97,108.91) .. (255.43,102.43) .. controls (255.47,101.91) and (255.72,82.05) .. (259.43,81.43) .. controls (265.64,80.39) and (270.98,82.83) .. (274.43,87.43) .. controls (274.94,88.11) and (276.86,93.37) .. (277.43,93.43) .. controls (283.76,94.13) and (297.41,94.3) .. (298.43,102.43) .. controls (299.87,113.93) and (286.06,117.88) .. (294.43,130.43) ;
%Shape: Free Drawing [id:dp6403818711667688] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=0.75] [line join = round][line cap = round] (257.43,135.43) .. controls (252.57,135.43) and (253.3,118.75) .. (253.43,117.43) .. controls (253.66,115.13) and (257.69,114.11) .. (260.43,113.43) .. controls (266.46,111.92) and (268.43,100.57) .. (278.43,103.43) .. controls (290.14,106.78) and (277.87,118.22) .. (277.43,124.43) .. controls (277.12,128.75) and (277.1,133.11) .. (277.43,137.43) .. controls (277.74,141.49) and (293.86,142.94) .. (297.43,142.43) .. controls (304.28,141.45) and (307.43,134.68) .. (307.43,128.43) ;
%Shape: Circle [id:dp16142511067198195] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (131,138) .. controls (131,137.45) and (131.45,137) .. (132,137) .. controls (132.55,137) and (133,137.45) .. (133,138) .. controls (133,138.55) and (132.55,139) .. (132,139) .. controls (131.45,139) and (131,138.55) .. (131,138) -- cycle ;
%Shape: Circle [id:dp3430388823901913] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (257,136) .. controls (257,135.45) and (257.45,135) .. (258,135) .. controls (258.55,135) and (259,135.45) .. (259,136) .. controls (259,136.55) and (258.55,137) .. (258,137) .. controls (257.45,137) and (257,136.55) .. (257,136) -- cycle ;
%Shape: Circle [id:dp05758642157009719] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (294,130) .. controls (294,129.45) and (294.45,129) .. (295,129) .. controls (295.55,129) and (296,129.45) .. (296,130) .. controls (296,130.55) and (295.55,131) .. (295,131) .. controls (294.45,131) and (294,130.55) .. (294,130) -- cycle ;
%Shape: Circle [id:dp6693742833406049] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (307,129) .. controls (307,128.45) and (307.45,128) .. (308,128) .. controls (308.55,128) and (309,128.45) .. (309,129) .. controls (309,129.55) and (308.55,130) .. (308,130) .. controls (307.45,130) and (307,129.55) .. (307,129) -- cycle ;

% Text Node
\draw (198,152) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X$};
% Text Node
\draw (184,103.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{S}$};
% Text Node
\draw (142,131.4) node [anchor=north west][inner sep=0.75pt]    {$I$};
% Text Node
\draw (323,152) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X$};
% Text Node
\draw (309,103.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{S}$};
% Text Node
\draw (268,132.4) node [anchor=north west][inner sep=0.75pt]    {$I$};
% Text Node
\draw (128,121.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$t_{0}$};
% Text Node
\draw (255,119.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$t_{0}$};
% Text Node
\draw (160,90.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$t_{\infty }$};
% Text Node
\draw (294,112.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$t_{T}$};
\end{tikzpicture}

==> graphics/safety2.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1.2,xscale=1.2]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp0044176096267762865] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (102,69.43) -- (215.43,69.43) -- (215.43,171.43) -- (102,171.43) -- cycle ;
%Shape: Polygon [id:ds5309575007412408] 
\draw  [fill={rgb, 255:red, 228; green, 239; blue, 214 }  ,fill opacity=1 ] (151.43,75.43) -- (211,103) -- (171,164) -- (119.43,155.43) -- (111,106) -- cycle ;
%Shape: Ellipse [id:dp45235881723985827] 
\draw  [fill={rgb, 255:red, 230; green, 242; blue, 249 }  ,fill opacity=1 ] (128.55,152.44) .. controls (112.28,139.43) and (110.39,114.76) .. (124.32,97.35) .. controls (138.25,79.94) and (162.73,76.37) .. (178.99,89.38) .. controls (195.26,102.39) and (197.15,127.06) .. (183.22,144.47) .. controls (169.29,161.88) and (144.81,165.45) .. (128.55,152.44) -- cycle ;
%Shape: Circle [id:dp7183588582096849] 
\draw  [fill={rgb, 255:red, 240; green, 225; blue, 254 }  ,fill opacity=1 ] (126.43,132.93) .. controls (126.43,123.26) and (134.26,115.43) .. (143.93,115.43) .. controls (153.59,115.43) and (161.43,123.26) .. (161.43,132.93) .. controls (161.43,142.59) and (153.59,150.43) .. (143.93,150.43) .. controls (134.26,150.43) and (126.43,142.59) .. (126.43,132.93) -- cycle ;

% Text Node
\draw (198,152) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X$};
% Text Node
\draw (192,98.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{S}$};
% Text Node
\draw (140,125.4) node [anchor=north west][inner sep=0.75pt]    {$I$};
% Text Node
\draw (167,107.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{B}$};

\end{tikzpicture}

==> sections_new/problem_new.tex <==
\section{Problem setup}
\subsection{System dynamics and uncertainty description}
Consider a controlled stochastic discrete-time system
\begin{equation}\label{eq:poly:sys}
x_{t+1} = A(x_t)x_t + B(x_t)u_t(x_t) + w_t,
\end{equation}
where $A(x): \mathbb{R}^n \rightarrow \mathbb{R}^{n \times n}, B(x):\mathbb{R}^n \rightarrow \mathbb{R}^{n \times m}$ are polynomial matrices\footnote{This is w.l.o.g. as general input-affine systems of the form $x_{t+1} = f(x_t) + g(x_t)u_t(x_t)$ can always be written as in \eqref{eq:poly:sys} via suitable algebraic manupulations.}, $u_t(x_t)$ is a control law (to be designed), and $w_t$ is a stochastic disturbance.  We assume that the initial state $x_0$ is fixed to an arbitrary vector $x \in \mathbb{R}^n$.\footnote{More precisely, we assume that the distribution of $x_0$ is the Dirac measure
concentrated at $x_0 \in \mathbb{R}^n$.} Systems of the form \eqref{eq:poly:sys} are referred to as (stochastic) \textit{input-affine polynomial} systems and find broad applications in robotics, medicine, and autonomous vehicles. 

We define the setup for the reminder of the paper. Let $(\Omega, \mathcal{F}, {\mathbb{P}})$ be the probability space for the disturbance affecting  \eqref{eq:poly:sys}. In particular, we have the probability measure $\mathbb{P}(w_t \in F)\coloneqq \mathbb{P}(\{\omega \in \Omega : w_t(\omega) \in F\})$. For $t \geq 0$ let $w_t:\Omega \rightarrow \mathbb{W} \subseteq \mathbb{R}^d$ be a sequence of independent, identically distributed (i.i.d.) real-valued random variables. Thus, $w_t^{-1}(F) \coloneqq \{\omega \in \Omega : w_t(\omega) \in F\} \in \mathcal{F}$ for each $F \in \mathbf{B}(\mathbb{W})$. Consider now the sequence $\mathbf{w}_\infty: \Omega \rightarrow \mathbb{W}^\infty$, $\mathbf{w}_\infty = \{w_t\}_{t=0}^\infty$ and let $(\mathcal{F}_0, \mathcal{F}_1,\ldots)$ denote its natural filtration. That is, $\mathcal{F}_t \subset \mathcal{F}$ consists on all sets of the form $\{\omega \in \Omega \: : \: \mathbf{w}_{[:t]} \in F\}$ for $F \in \mathbf{B}(\mathbb{W}^t)$, where $\mathbf{w}_{[:t]}:\Omega \rightarrow \mathbb{W}^{t+1}, \mathbf{w}_{[:t]} = (w_0, w_1,\ldots, w_{t})$ is a subsequence. Informally speaking, $\mathcal{F}_t$ corresponds to the information available up to time $t$. For $1\le p \leq \infty$, let $\mathcal{L}_t^p$ denote the space of $\mathcal{F}_t$-measurable random variables $\mathbf{w}_{[:t]}$ with finite $p$-th moment, i.e., $\left(\mathbb{E}(|\mathbf{w}_{[:t]}|^p)\right)^{\frac{1}{p}} < +\infty$. In this work, we will focus on the case $p=1$ to ease presentation. Each random variable has an equivalent probability measure $\mu:\mathbf{B}(\mathbb{W}) \rightarrow [0,1]$ defined as $\mu(F) = \mathbb{P}(\{\omega \in \Omega : w_t(\omega) \in F\})$ for all $F \in \mathbf{B}(\mathbb{W}), \: t \geq 0$. We consider the following standing assumption.

\begin{assumption}[Disturbance model]\label{ass:noise:new}
$\mathbb{W}$ is compact and contains the origin in its interior. Additionally $\mu$ has finite second moment.
\end{assumption}

%Assumption \eqref{ass:noise:new} is satisfied, for example, by Sub-Gaussian distributions and trivially when $\mathbb{W}$ is compact.
Assumption \eqref{ass:noise:new} implies that $\mu$ satisfies an exponential moment bound, i.e., there exist $a_1> 1, a_2 > 0, M > 0$ such that $\mathbb{E}[\text{exp}(a_2 |w|^{a_1})] < M < \infty$.

The dynamical equation in \eqref{eq:poly:sys} gives rise to a random process. We define a random process $\mathbf{x}$ as the sequence of random variables $x_t: \text{dom}(x_i) \subset \Omega \rightarrow \mathbb{R}^d$ and $\text{dom}(x_{t+1}) \subset \text{dom}(x_i)$. The random process $\mathbf{x}$ is \textit{adapted} to the natural filtration of $\mathbf{w}$ if $x_{t+1}$ is $\mathcal{F}_t$ measurable for each $t \geq 0$., i.e., if $x_{t+1}(\omega) = A(x_t(\omega)) x_t(\omega) + B(x_t(\omega)) u(x_t(\omega)) + w_t(\omega)$ for all $\omega \in \text{dom}(x_{t+1})$ and $t \geq 0$\footnote{Polynomials are continuous functions, therefore measurable. This ensures the well-posedness of our problem formulation.}. We use $x(t+1,x_0,\mathbf{w}_{[:t]})$ to denote the random solution of \eqref{eq:poly:sys} given the deterministic initial condition $x_0$, i.e., $x_0(\omega) = x_0$ for all $\omega \in \Omega$, with $x_0 \in \mathcal{I}$.

 





% In line with Subsection \eqref{prelim:safety}, we turn the stochastic safety verification problem into an existence problem and look for an invariant set for \eqref{eq:poly:sys}. Given a Borel measurable function $b(x)$, we define the conditional expected value as
% $$
% \begin{aligned}
% & \mathbb{E}[b(x(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t}](\omega) \coloneqq \\
% & \quad \int_{\mathbb{W}}b(x(t+1, x_0, (w_0(\omega),\ldots, w_{t-1}(\omega),w)\mu(dw).
% \end{aligned}
% $$

% Consequently, we might consider the following stochastic safety definition.
% \begin{definition}[Risk-neutral Invariant Set]\label{def:invariance:stoch}
% The set $\mathcal{B} \coloneqq \{x \in \mathbb{R}^n\; : \; b(x) \geq 0\} \subset \mathbb{R}^n$ is an \emph{invariant set in expecation} for the stochastic system $x_{t+1} = A(x_t)x_t + B(x_t)u(x_t) + w_t$ if, for any $x_0 \in \mathcal{B}$ and $t \geq 0$, it holds 
% $$\mathbb{E}[b({x}(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t}](\omega) \geq 0, \;\; \forall t \geq 0.$$
% \end{definition}
% \smallskip
% Clearly, whenever $\mathcal{B} \subseteq \mathcal{S}$, Definition \ref{def:invariance:stoch} implies $\mathbb{E}[s_j({x}(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t-1}](\omega) \geq 0, \; j = 1,\ldots,q, \;\; \forall t \geq 0$. We refer to this property as \textit{risk-neutral safety}, and we call $b(x)$ a \textit{stochastic control barrier function}.


% However, the expectation operator cannot account for the variability of stochastic system behaviors. Leveraging the theory of risk functionals, we aim to define a generalized notion of safety for stochastic discrete-time systems, where the generality pertains to the ways in which the distribution of the control barrier function can be characterized. We introduce the necessary background on risk functionals in the following.

%of real-valued random variables affecting, with $w_t : \Omega \rightarrow \mathbb{W} \subseteq \mathbb{R}$. We define the subsequence $\mathbf{w}_{[:t]}:\Omega \rightarrow \mathbb{W}^t$ as $\mathbf{w}_{[:t]} = (w_0, w_1,\ldots, w_{t-1})$. 




\subsection{Safety requirements}

% We consider the stochastic discrete-time input-affine polynomial system in \eqref{eq:poly:sys} and let the following assumption hold true throughout.
 
% \begin{assumption}[Disturbance model]\label{ass:noise}
% The disturbances $w_t: \Omega \rightarrow \mathbb{W}$ are independent and identically distributed (i.i.d.) in time random variables with finite $p-$th moment. The support $\mathbb{W} \subseteq \mathbb{R}^d$ is compact and contains the origin. Each random variable has an equivalent probability measure $\mu:\mathcal{B}(\mathbb{W}) \rightarrow [0,1]$ defined such that $\mu(F) = {P}(\{\omega \in \Omega : w_t(\omega) \in F\})$ for all $F \in \mathcal{B}(\mathbb{W}), \: t \geq 0$. Furthermore, $\mu$ satisfies an exponential moment bound, i.e., there exist $\beta > 1, \gamma > 0, M > 0$ such that $\mathbb{E}[\text{exp}(\gamma |w|^\beta)] < M < \infty$.
% \end{assumption}

% The exponential moment bound requirement is satisfied, for example, by Sub-Gaussian distributions and trivially by compactly supported distributions.

%  Let us denote as $x(t+1, x_0,\mathbf{w}_{[:t]})$  the solution of the closed-loop system $x_{t+1} = A(x_t)x_t + B(x_t) u(x_t) + w_t$ at time $t+1$ starting from the initial condition $x_0 \in \mathcal{I} \subseteq \mathcal{S}$ under the random sequence $\mathbf{w}_{[:t]}$. As a result the closed-loop state $x(t+1, x_0,\mathbf{w}_{[:t]})$ is itself a random variable.

% Under Assumption \ref{ass:noise}, whenever the probability measure of the i.i.d. random variables $(w_0, \ldots, w_{t-2})$ is known, their joint distribution measure $\mu^{t-1}:\mathcal{B}(\mathbb{W}^{t-1}) \rightarrow [0,1]$ is 
% $$
% \mu^{t-1}(F) = \mu(F_0)\mu(F_{1})\ldots \mu(F_{t-2}),
% $$for all $F = (F_0, F_{1}\ldots F_{t-2}) \in \mathcal{B}(\mathbb{W}^{t-1})$, where $t \in \mathbb{N}$.  For the Borel measurable functions $b(x)$, we can define the conditional expected value as
% $$
% \begin{aligned}
% & \mathbb{E}[b(x(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t-1}](\omega) \coloneqq \\
% & \quad \int_{\mathbb{W}}b(x(t+1, x_0, (w_0(\omega),\ldots, w_{t-2}(\omega),w)d\mu(\omega).
% \end{aligned}
% $$

% Consequently, one might seamlessly extend the definition of control invariant set in Definition \ref{def:invariance} for discrete-time stochastic systems of the form \eqref{eq:poly:sys} as follows.
% \begin{definition}[Risk-neutral Invariant Set]\label{def:invariance:stoch}
% The set $\mathcal{B} \coloneqq \{x \in \mathbb{R}^n\; : \; b(x) \geq 0\} \subset \mathbb{R}^n$ is an \emph{invariant set in expecation} for the stochastic system $x_{t+1} = A(x_t)x_t + B(x_t)u(x_t) + w_t$ if, for any $x_0 \in \mathcal{B}$ and $t \geq 0$, it holds 
% $$\mathbb{E}[b({x}(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t-1}](\omega) \geq 0, \;\; \forall t \geq 0.$$
% \end{definition}

% Clearly, whenever $\mathcal{B} \subseteq \mathcal{S}$, Definition \ref{def:invariance:stoch} implies $\mathbb{E}[s_j({x}(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t-1}](\omega) \geq 0, \; j = 1,\ldots,q, \;\; \forall t \geq 0$. We refer to this property as \textit{risk-neutral safety}, and we call $b(x)$ a \textit{stochastic control barrier function}.


% However, the expectation operator cannot account for the variability of stochastic system behaviors. Leveraging the theory of risk functionals described in Subsection \ref{sec:risk:measures}, we define a generalized notion of safety for stochastic discrete-time systems, where the generality pertains to the ways in which the distribution of the control barrier function can be characterized. 
We focus on safety requirements that are formulated as constraints on the system states as $x_t \in \mathcal{S}, \forall t \geq 0$, where the \textit{safe} set $\mathcal{S}$ is defined as:
\begin{equation}\label{eq:poly:set}
\mathcal{S}\coloneqq \bigcap_{j=1}^q \{x \in \mathbb{R}^n \; : \; s_j(x) \geq 0\},
\end{equation}
for given application-specific polynomials $s_1(x),\ldots, s_q(x)$. Semi-algebraic safe sets virtually encompass all safety specifications of engineering systems. We further consider a semi-algebraic initial set $\mathcal{I} \subseteq \mathcal{S}$ defined as
\begin{equation}\label{eq:poly:set:init}
\mathcal{I}\coloneqq \bigcap_{j=1}^q \{x \in \mathbb{R}^n \; : \; r_j(x) \geq 0\}.
\end{equation}


Given system \eqref{eq:poly:sys}, a safe set \eqref{eq:poly:set} and an initial set \eqref{eq:poly:set:init}, we aim to assess whether the random solution of \eqref{eq:poly:sys}, i.e., $x(t+1,x_0,\mathbf{w}_{[:t]})$,  satisfies a generalized notion of stochastic safety that is based on the theory risk functionals. More precisely, we consider the class of coherent risk measures, namely maps $\rho: \Omega \rightarrow \mathbb{R}$ that possess desirable properties and a dual representation. We collect the necessary background material on risk measures in Appendix \ref{sec:risk:measures}.

Leveraging the risk functionals formalism, we outline our definition of risk-aware safety. We distinguish between the infinite-horizon case and the finite-horizon case.

\smallskip
\subsubsection{Infinite-horizon case} We consider the following generalized definition of safety.
\begin{definition}[$\rho$-risk-aware safety]\label{def:riskaware:safety}
Consider a stochastic system $x_{t+1} = F(x_t, w_t)$, the safe set $\mathcal{S}$, and a set of initial conditions $\mathcal{I}$. For any $x_0 \in \mathcal{I} \subseteq \mathcal{S}$, consider the following condition:
\begin{equation*}
\rho\left[\bigcap_{j=1}^q s_j\left(x(t,x_0, \mathbf{w}_{[:t-1]})\right)|\mathcal{F}_{t-1}\right] \leq c, \quad \forall t \geq 0.
\end{equation*}
If $c = 0$ then, then we say the system is $\rho$-risk-aware safe. If $c >  0$, then we say the system is noise-to-state $\rho-$risk aware safe and we term $c$ the safety margin.
\end{definition}


% Consider a compact set $\mathcal{B}$ defined as the zero super-level set of a continuous function $b(x)$, i.e.,
% \begin{equation}\label{eq:B:set}
% \mathcal{B} = \{ x | b(x) \geq 0\}.
% \end{equation}
% The set $\mathcal{B}$ is an invariant set for \eqref{eq:det:system} if 
% \begin{equation}\label{eq:safety:informal}
% \forall x \in \mathcal{B}, \; \text{it holds} \;\;  b(f(x)) \geq 0.
% \end{equation}


% A standard condition for the requirement in Definition \ref{def:invariance} to hold is provided next.
% \begin{lemma}[Sufficient condition for safety]\label{lemma:det:sys}
% If there exists an extended class-$\mathcal{K}$ function $\alpha(\cdot)$, with $\alpha(s) < s$ for $s > 0$, such that
% $
% b(F(x)) - b(x) + \alpha(b(x)) \geq 0, 
% $
% then $\mathcal{B} \coloneqq \{x \in \mathbb{R}^n\; :\; b(x) \geq 0\}$ is an invariant set for system $x_{t+1} = F(x_t)$.
% \end{lemma}

%Recall that in view of Definition \ref{def:risk_measures}, it is intuitive to associate a low risk to realizations $\tilde{x}$ such that $b(\tilde{x})$ is a large positive value, and, vice-versa, a large risk to those realizations leading to $b(\tilde{x})$ being a large negative value. 



% Equipped with a way to assess the riskiness of $b(x_t)$, we can now state our notion of risk-aware safety.

% \begin{definition}[Risk-aware safety]\label{def:stochastic:safety}
% The set $\mathcal{B} \coloneqq \{x \in \mathbb{R}^n\; : \; b(x) \geq 0\} \subset \mathbb{R}^n$ is an \emph{invariant set with respect to the risk measure $\rho$} for the stochastic system $x_{t+1} = A(x_t)x_t + B(x_t)u(x_t) + w_t$ if, for any $x_0 \in \mathcal{B}$ and $t \geq 0$, it holds 
% $$\rho[b({x}(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t-1}](\omega) \leq 0, \;\; \forall t \geq 0.$$

% Whenever $\mathcal{B} \subseteq \mathcal{S}$, the following implication holds true:
% $$\rho[s_j({x}(t+1, x_0,\mathbf{w}_{[:t]}))|\mathcal{F}_{t-1}](\omega) \leq 0, \; j = 1,\ldots,q, \;\; \forall t \geq 0.$$ We refer to this property as \textit{risk-neutral safety w.r.t. $\rho$}.
% \end{definition}

\smallskip
\subsubsection{Finite-time case} Whenever the time horizon of our safety verification problem is finite (but possibly large), a notion of \textit{safety in probability} is preferable, where the entire shape of the probability distribution concurs in determining the safety specification. %Similarly as before, we can exploit the relationship between invariant set and safety verification problem as follows.


\begin{definition}[$T-$step Exit Probability]\label{def:finite:safety}
Consider a stochastic system $x_{t+1} = F(x_t, w_t)$, the safe set $\mathcal{S}$, and a set of initial conditions $\mathcal{I}$. For any $T \in \mathbb{N}, \; \gamma \in \mathbb{R}_{\geq 0}$ and $x_0 \in \mathcal{I} \subseteq \mathcal{S}$, the $T-$step exit probability of \eqref{eq:poly:sys} is defined as
$$
\mathbb{P}_{\text{exit}}(T, \gamma, x_0)\!=\!\mathbb{P}\!\left(\!\min_{t \in [0,\ldots,T]} \bigcap_{j=0}^q s_j\left({x}(t, x_0,\mathbf{w}_{[:t-1]})\right) < -\gamma \!\right)\!.
$$
\end{definition}
Equation \eqref{def:finite:safety} described the probability that \eqref{eq:poly:sys} leaves the $\gamma$-superlevel set of $\bigcup_{j=1}^qs_j(x)$ within $T$ timesteps. Notice that this definition is only applicable to cases where $T$ is finite: for the infinite-horizon case in the presence of unbounded noise it holds $\mathbb{P}_{\text{exit}}(T, \gamma, x_0)=1$, making the analysis vacuous. 

\begin{definition}[$\alpha$-safety in probability]\label{def:finite:safety}
Consider a stochastic system $x_{t+1} = F(x_t, w_t)$, the safe set $\mathcal{S}$, and a set of initial conditions $\mathcal{I} \subseteq \mathcal{S}$. For any $T \in \mathbb{N}, \; \gamma \in \mathbb{R}_{\geq 0}$ and $x_0 \in \mathcal{I}$, if the stochastic system $x_{t+1} = F(x_t, w_t)$ satisfies 
$
1 - \mathbb{P}_{\text{exit}}(T, 0, x_0)  \geq \alpha$ for $\alpha \in (0,1)$, we say that it is $\alpha$-safe in probability.
\end{definition}

\subsection{Problem formulation and overview}
We propose to employ the framework of CBFs together with the theory of risk functionals as a principled way to certify safety of stochastic discrete-time dynamical systems. Ultimately, our problem formulation is as follows.

\begin{problem}
Given system \eqref{eq:poly:sys}, a safe set \eqref{eq:poly:set}, an initial set \eqref{eq:poly:set:init} and an existing well-performing  controller $u_{\text{nom}}(\cdot)$, design a risk-aware safety filter to enhance the safety guarantees of $u_{\text{nom}}(\cdot)$ according to either Definition \eqref{def:riskaware:safety} (for the infinite-time case) or Definition \eqref{def:finite:safety} (for the finite-time case). 
\end{problem}

In particular, we require the applied control law to meet prescribed input constraints of the form $u(x) \in \mathcal{U} \subseteq \mathbb{R}^m$ and to produce control action with certain regularity properties, i.e., to avoid undesired chattering that can lead to system malfunction. As mentioned in the introduction, the design of a suitable CBF and of its associated controller is a challenging non-convex task, which is here further complicated by the addition of the risk functional map. To tackle the problem in a computationally efficient manner, we decompose the task into the three steps listed in Subsection \eqref{sec:contribution}, whose interconnections are reported in Figure \ref{fig:blocks}. In the sequel, we will describe each step.
% \end{itemize}

\begin{figure*}[!htb]
\centering
%\includegraphics[width=\linewidth]{graphics/placeholder.png}



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp07239426359409529] 
\draw   (32,43) -- (120,43) -- (120,83) -- (32,83) -- cycle ;
%Shape: Rectangle [id:dp883683339642827] 
\draw   (171,43) -- (259,43) -- (259,83) -- (171,83) -- cycle ;
%Shape: Rectangle [id:dp5188243030693593] 
\draw   (310,43) -- (398,43) -- (398,83) -- (310,83) -- cycle ;
%Straight Lines [id:da7049231314831021] 
\draw    (120,62) -- (168,62) ;
\draw [shift={(171,62)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da40441368427724855] 
\draw    (259,63) -- (307,63) ;
\draw [shift={(310,63)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da7062296569592217] 
\draw    (356,128.6) -- (356,132) ;
\draw [shift={(356,135)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Rectangle [id:dp3957950785101547] 
\draw   (293,135) -- (426,135) -- (426,175) -- (293,175) -- cycle ;
%Shape: Rectangle [id:dp6710013249423419] 
\draw   (462,135) -- (621,135) -- (621,175) -- (462,175) -- cycle ;
%Straight Lines [id:da06935176722837233] 
\draw    (426,155) -- (459,155) ;
\draw [shift={(462,155)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Rectangle [id:dp03338520745356166] 
\draw   (188,136) -- (247,136) -- (247,176) -- (188,176) -- cycle ;
%Straight Lines [id:da7553776706429445] 
\draw    (247,147) -- (291,147) ;
\draw [shift={(294,147)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da7172430062348256] 
\draw    (161,155) -- (186,155) ;
\draw [shift={(189,155)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da5030624546323494] 
\draw    (161,155) -- (161,203) ;
%Straight Lines [id:da6939409050260672] 
\draw    (161,203) -- (645,203) ;
%Straight Lines [id:da9785412328550411] 
\draw    (645,155) -- (645,203) ;
%Straight Lines [id:da8018822444925917] 
\draw    (622,155) -- (645,155) ;
%Straight Lines [id:da13201029844109247] 
\draw    (267,164) -- (267,203) ;
\draw [shift={(267,203)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da12655912507632494] 
\draw    (267,164) -- (290,164) ;
\draw [shift={(293,164)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da6119595336073151] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (22,91) -- (646,91) ;
%Straight Lines [id:da27845773631466897] 
\draw    (356,83) -- (356,118.6) ;

% Text Node
\draw (75.01,32.8) node  [font=\footnotesize] [align=left] { \textbf{Nominal synthesis}};
% Text Node
\draw (200.01,32.8) node  [font=\footnotesize] [align=left] { \ \ \ \ \ \ \ \ \textbf{Risk-aware analysis}};
% Text Node
\draw (353.01,32.8) node  [font=\footnotesize] [align=left] { \textbf{Implementation}};
% Text Node
\draw (75,63) node  [font=\footnotesize] [align=left] { SOS Program};
% Text Node
\draw (215,63) node  [font=\footnotesize] [align=left] { Noise-to-state};
% Text Node
\draw (354,63) node  [font=\footnotesize] [align=left] { Design CP};
% Text Node
\draw (126,47) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$b^{\star }( x) \ $};
% Text Node
\draw (125,64) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\pi ^{\star }( x)$};
% Text Node
\draw (358,95) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\mathcal{H}_{\rho }( x)$};
% Text Node
\draw (268,48) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$b_{\rho }( x) \ $};
% Text Node
\draw (304,143) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\min_{u} \ \ \ell ( u,\ u_{\text{nom}}( x_{t}))$};
% Text Node
\draw (317,155) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\text{s.t.} \ \ \ u\ \in \mathcal{H}_{\rho }( x_{t})$};
% Text Node
\draw (468,148) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$x_{t+1} \ =\ f\left( x_{t} ,u^{\star }( x_{t})\right) \ +\ w_{t}$};
% Text Node
\draw (213,120.02) node  [font=\footnotesize] [align=left] { Nominal controller};
% Text Node
\draw (528.01,122.8) node  [font=\footnotesize] [align=left] { \ \ \ \ \ \ \ \ System};
% Text Node
\draw (626,140) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$x_{t}$};
% Text Node
\draw (195,148) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$u_{\text{nom}}( x_{t})$};
% Text Node
\draw (628.01,80.8) node  [font=\footnotesize] [align=left] { Offline};
% Text Node
\draw (628,100.8) node  [font=\footnotesize] [align=left] { Online};
% Text Node
\draw (345.01,122.8) node  [font=\footnotesize] [align=left] { \ \ \ \ \ \ \ \ Risk-aware safety filter};


\end{tikzpicture}
\caption{Block diagrams of the proposed end-to-end design of risk-aware safety filters. The paper focuses on the components highlighted in bold.}
\label{fig:blocks}
\end{figure*}

% \begin{enumerate}
% \item Section \ref{sec:synthesis}: Convex co-design of CBFs and safe feedback control under input constraints for the nominal counterpart.
% \item Section \ref{sec:risk:measures}: Noise-to-state risk-aware safety.
% \item Section \ref{sec:implementation}: Implementation.
% \end{enumerate}


==> sections_new/synthesis_new.tex <==
\section{Co-design of CBFs and state feedback controllers}\label{sec:main}
In this section, we propose convex formulations to co-design a CBF $b(x)$ and a safe feedback controller $u(x)$ for system \eqref{eq:poly:sys} for different geometric shapes of the initial set $\mathcal{I}$ and safe set $\mathcal{S}$. We shall consider the following parametrization:
\begin{subequations}\label{eq:parametrization:all}
\begin{align}
b(x) & = 1 - x^\top \Omega^{-1}x,\\
u(x) & = Y \Omega^{-1}x
\end{align}
\end{subequations}
where $\Omega \in \mathbb{R}^{n \times n}, Y \in \mathbb{R}^{m \times n}$ are matrices to be designed. Notice that higher-order CBFs would allow to accommodate systems of arbitrary (high) relative degrees; however, they suffer from two drawbacks. First, they return a nonlinear design problem, which cannot be convexified. Second, they require to (numerically) compute the high-order moments of the noise probability distribution, which may be computationally expensive. As a result, we proceed with a quadratic parametrization for $b(x)$ as it allows a good compromise between expressivity and computational tractability.

To ease presentation, we derive our main result based on a specific geometry of $\mathcal{S}$ and $\mathcal{I}$ and later extend it.
\vspace{-0.2cm}
\begin{assumption}[Initial and safe set]\label{ass:sets}
$\mathcal{S}$ is non-empty, and
 $s_j(x)=a_j^\top x+1,j=1,\ldots,q.$ Further, $\mathcal{I} = \{ x | 1 - x^\top R x \geq 0\}$ for a given $R = R^\top \succ 0$.
\end{assumption}
\vspace{-0.2cm}
We defer all proofs to the Appendix.
\vspace{-0.2cm}

\subsection{Design for bounded disturbances}\label{section:infinite}
We consider uncertain systems as in \eqref{eq:poly:set}, driven by additive noise $w$ supported on $\mathbb{W}\subseteq \mathbb{R}^n$. We assume the following structure for the support set and further generalize it in Section 4.3.

\begin{assumption}[Bounded support]\label{eq:support}
The disturbance is bounded in $\mathbb{W}:= \{ w \in \mathbb{R}^n : w^\top w \leq 1\}$.
\end{assumption}

When confronted with disturbances, we naturally revise the forward invariance condition in \eqref{eq:increase} as
\begin{equation}\label{eq:robust:c1}
(w^\top w \leq 1) \wedge (x \in \mathcal{B}) \implies (Ax + Bu(x) + Dw) \in \mathcal{B}.
\end{equation}
A \textit{sufficient} condition for \eqref{eq:robust:c1} to hold is provided by the following \textit{global} implication: For all $x \in \mathbb{R}^n$ and a fixed $\beta \in (0,1)$, it holds
\vspace{-0.2cm}
\begin{equation}\label{eq:robust:c2}
(w^\top w \leq 1) \implies b(Ax + Bu(x) + Dw) - b(x) \geq -\beta b(x).
\end{equation}
Despite providing a conservative approximation of \eqref{eq:robust:c1}, \eqref{eq:robust:c2} allows for a convex reformulation, as shown next. Fix $\lambda, \beta \in (0,1)$ and let $\tilde{\beta} = 1 - \beta \in (0,1)$. Further, consider the following \textit{jointly convex} optimization problem:


\begin{subequations}\label{eq:convex-without-input-constraints}
\begin{align}
    \max~&\mathrm{log det}(\Omega)\\
    \mathrm{s.t.}~&  Y \in\mathbb{R}^{m\times n},  0\prec\Omega=\Omega^\top\in\mathbb{R}^{n\times n}, \\ 
    &\begin{bmatrix}
        -\tilde{\beta} \Omega + \lambda \Omega & 0 & \Omega A^\top + Y^\top B^\top \\
        0 & -\lambda I & D^\top\\
        A\Omega + BY & D & -\Omega
    \end{bmatrix} \preceq 0,\label{eq:convex-e}\\
     &\begin{bmatrix}
     R&I\\I&\Omega
     \end{bmatrix}\succeq 0,\label{eq:convex-f}\\
    &1-a_j^\top \Omega a_j\geq 0,\: j=1,\ldots,q,\label{eq:convex-h}
\end{align}
\end{subequations}
where $\Omega$, $Y$ are decision variables. We show next that \eqref{eq:convex-without-input-constraints} provides a convex design procedure for the synthesis of a valid CBF and feedback controller for \eqref{eq:poly:sys}, certifying infinite-horizon safety according to Definition \eqref{def:bounded:safety}. 

\begin{tcolorbox}[colback=purple!6, colframe=white, sharp corners=south, boxrule=0pt,boxsep=-0.5mm]
\begin{theorem}\label{th:convex-design}
    Consider system \eqref{eq:poly:sys}, safe set $\mathcal{S}$, and initial set $\mathcal{I}$. Let Assumptions \eqref{ass:noise} and \ref{ass:sets} hold, and $\mathcal{U}=\mathbb{R}^m$. Assume that for a fixed $\lambda \in (0,1)$ a solution to \eqref{eq:convex-without-input-constraints} exists and is denoted by $\Omega,R,Y,\{\sigma_j\}_{j=1}^q$. Set $u = u(x)=Y\Omega^{-1}x$ and define $\mathcal{B} = \{ x \in \mathbb{R}^n \; : \; 1 - x^\top \Omega^{-1}x \geq 0\}$. Then the following hold
    \begin{enumerate}
        \item $\mathcal{B}$ is an invariant set for $x_{t+1} =Ax_t+Bu(x_t) + Dw$.
        \item $\mathcal{I}\subseteq \mathcal{B}\subseteq\mathcal{S}$.
        \item $\mathcal{B}$ is the largest set satisfying 1) and 2) given the parametrization in \eqref{eq:parametrization:all}.
    \end{enumerate}
    Further, system \eqref{eq:poly:sys} under $u(x)$ is safe according to Definition \eqref{def:bounded:safety}.
\end{theorem}
\end{tcolorbox}
Note that the objective function in \eqref{eq:convex-without-input-constraints} can be substituted by $\max \mathrm{Tr}(\Omega)$, that is better supported by available solvers.


\begin{remark}[On optimizing over $\lambda$]
Recall that the described procedure presumes a fixed $\lambda \in (0,1)$. If the control designer wants to optimize over $\lambda$ as well, constraint \eqref{eq:convex-e} becomes non-convex due to the existence of the bilinear matrix term $\lambda \Omega$. Let $g(\lambda)$ denote the optimal value of \eqref{eq:convex-without-input-constraints} for a fixed value of $\beta$ (and hence $\tilde{\beta}$). We immediately notice that $g(\lambda)$ is not well-defined for $\lambda\leq 0$ or $\lambda \geq 1$ as the optimization program becomes infeasible (see also proof of Theorem \eqref{th:convex-design}). When $\lambda \in (0,1)$, $g(\lambda)$ can be showed to be quasi-convex. Thus, the optimization over $\lambda$ can be efficiently carried out by bisection on $(0,1)$ to find $\max_\lambda g(\lambda)$.  A similar reasoning can be carried out with respect to $\beta \in (0,1)$.
\end{remark}

 Finally, note that in the case of ellipsoidal safe set of the form $\mathcal{S} = \{ x \in \mathbb{R}^n \; \; 1 - x^\top S x \geq 0\}$ with $S \succ 0$ given, the containment condition $\mathcal{B} \subseteq \mathcal{S}$ in \eqref{eq:convex-h} boils down to
$$
\begin{aligned}
& \{x \in \mathbb{R}^n \:| \: 1 - x^\top \Omega^{-1}x \geq 0\} \subseteq \{x \in \mathbb{R}^n \:| \: 1 - x^\top S x \geq 0\}\\
& \hspace{2.7cm}\iff  \begin{bmatrix} \Omega & \Omega \\ \Omega &  S^{-1} \end{bmatrix} \succeq 0. 
\end{aligned}
$$

% {\color{blue} We conclude the section by showing how the presented framework fits the case of general nonlinear systems. Let $x_{t+1} = f(x_t, u_t) + Dw_t$, with $f$ being continuously differentiable. For some $\tilde{x} \in \mathbb{R}^n, \tilde{u} \in \mathbb{R}^m$ define 
% $$
% A_{\tilde{x}} = \frac{\partial f}{\partial x}\big|_{x = \tilde{x}}, \quad B_{\tilde{u}} = \frac{\partial f}{\partial u}\big|_{u = \tilde{u}}.
% $$
% Then the nonlinear system amounts to
% \begin{equation}
% x_{t+1} = A_{\tilde{x}} x_t + B_{\tilde{u}} u_t + D w_t,
% \end{equation}
% which is of the form of \eqref{eq:poly:sys} with time-varying systems matrices. QUESTION: do we assume $\tilde{x}, \tilde{u}$ to be exogenously given a prior (possibly time-varying as well?)? }


\subsection{Design for finite-horizon safety}\label{sec:design:finite}
We next consider the case of unbounded support $\mathbb{W}$. As already mentioned, in this case we relax our notion of safety to the requirement:
\begin{equation}\label{eq:safety:finite:recap}
\begin{aligned}
&\text{Pr}(x(t, x_0, \mathbf{w}_{[:t-1]}) \in \mathcal{S}, \forall t = \{0,\ldots,T\})\\
= & 1 - \text{Pr}\left(\min_{t \in \{0,\ldots,T\}} b_t(x(t, x_0, \mathbf{w}_{[:t-1]})) < 0 \right)\\
\geq & 1 - \alpha,
\end{aligned}
\end{equation}
for $\alpha \in (0,1)$ being a user-defined risk tolerance parameter. To encode \eqref{eq:safety:finite:recap} via a convex optimization problem, we shall exploit tools from martingale theory. 

Martingale theory allows us to provide sufficient conditions for \eqref{eq:safety:finite:recap} to hold in the form of constraints on the expected value of $b(\cdot)$ reading as
\begin{equation}\label{eq:safety:martingale}
\mathbb{E}[b(Ax_t + Bu(x_t) + w_t) | \mathcal{F}_{t-1}] - b(x_t) \geq -\beta b(x_t) - \delta,
\end{equation}
with $\beta \in (0,1), \delta \geq 0$, for all $t = \{0,\ldots, T\}$. Note that we introduce the decision variable $\delta$ in \eqref{eq:safety:martingale} to reduce the conservatism of the inequality and allow for an additional degree of freedom in the design. This construction relaxes the non-convexity\footnote{Recall that by definition $\text{Pr}(x \in \mathcal{S}) = \mathbb{E}_\mathbb{P}[1_{\mathcal{S}}(x)]$, where $1_{\mathcal{S}}(x) = 1$ if $x \in \mathcal{S}$, 0 otherwise. Clearly, $1_{\mathcal{S}}(x)$ is non-convex.} of the chance-constrained formulation in \eqref{eq:safety:finite:recap}.  Conversely, we show that the constraint in \eqref{eq:safety:martingale} is convex in the design variables $\Omega$ and $Y$ under Assumption \eqref{ass:noise}. Before providing our main result of this subsection, we describe the proposed procedure consisting of three main steps. First, by recognizing that $b(\cdot)$ might not have the desired martingale properties, we define a non-negative supermartingale $\zeta_t$ starting from the increase condition in \eqref{eq:safety:martingale} by shifting and scaling it appropriately. Second, by noticing that Ville's inequality (Lemma \eqref{lemma:Ville}) is now applicable to the constructed $\zeta_t$, we define a parameter $a^\star \in \mathbb{R}$ such that
$$
\left(\sup_{0 \leq t \leq T} \zeta_t \leq  a^\star \right) \implies \left( \inf_{0 \leq t \leq T} b(x_t) \geq 0 \right),
$$
in order to map the probabilistic guarantees back to the original system (e.g., in $b(\cdot)$). Third, armed with the bound derived from the previous step, we embed the condition in \eqref{eq:safety:martingale} into a convex optimization problem, while restricting the design to match with the user-defined maximum tolerance $\alpha$.





% Before outlining our proof, we collect some background and preliminary results.

% \begin{definition}[Supermartingale]\label{def:martingale}
% A discrete-time supermartingale is a discrete-time stochastic process $X_0, X_1,X_2,\ldots$ that satisfies the following two properties, for any time $t$: (i) $\mathbb{E}[|X_t|] < \infty$, and (ii) $\mathbb{E}[X_{t+1}|X_1, \ldots, X_{t}] \leq X_t$.
% \end{definition}
% Note that (ii) boils down to $\mathbb{E}[X_{t+1}| X_{t}] \leq X_t$ if $X_t$ evolves according to a Markovian dynamics.

% \begin{lemma}[Ville's inequality, \cite{ville1939etude}]\label{lemma:Ville}
% Let  $X_0, X_1,X_2,\ldots$ be a non-negative supermartingale. Then, for any  real $a > 0$,
% $$
% \emph{Pr}(\sup_{t \geq 0} X_t > a) \leq \frac{\mathbb{E}[X_0]}{a}.
% $$
% \end{lemma}

We consider each step individually. The following lemma shows how to construct a non-negative supermartingale starting from \eqref{eq:safety:martingale}.
\begin{lemma}\label{lemma:super}
Let $\beta \in (0,1), \delta \geq 0$, define $\psi = \beta + \delta \geq 0$, and pick $\eta \in (1,\frac{1}{1-\beta}]$ and $T \in \mathbb{N}, T < \infty$. Further, let $\Omega^{-1} \succ 0$ and assume \eqref{eq:safety:martingale} hold. Consider $$\zeta_t := \eta^t (x_t^\top \Omega^{-1} x_t) + \psi \eta \frac{\eta^T - \eta^t}{\eta - 1}.$$ Then, $\zeta_t$ is a non-negative supermartingale in the interval $ t = \{0,\ldots, T\}$.
\end{lemma}
% \begin{proof}
% Our goal is to construct a non-negative supermartingale $\zeta_t$ starting from \eqref{eq:safety:martingale}. To this end, note that \eqref{eq:safety:martingale} is equivalent to
% $$
% \mathbb{E}[x_{t+1}^\top \Omega^{-1}x_{t+1}] \leq \tilde{\beta} (x_t^\top \Omega^{-1} x_t) + \psi,
% $$
% for $\tilde{\beta} = 1 - \beta \in (0,1)$ and $\psi = 1 - \tilde{\beta} + \delta = \beta + \delta \geq 0$ by definition. By multiplying both sides of the previous inequality by $\eta^{t+1} > 0$ and adding the term $\psi \left(\sum_{i=1}^T \eta^{i} - \sum_{i=1}^{t+1} \eta^{i}\right)$ we get
% $$
% \begin{aligned}
% & \mathbb{E}\left[ \eta^{t+1}(x_{t+1}^\top \Omega^{-1}x_{t+1}) + \psi\left(\sum_{i=1}^T \eta^{i} - \sum_{i=1}^{t+1} \eta^{i} \right)\right] \\
% \leq & \eta^{t+1} \left(\tilde{\beta} (x_t^\top \Omega^{-1} z_t) + \psi\right)+ \psi \left(\sum_{i=1}^T \eta^{i} - \sum_{i=1}^{t+1} \eta^{i} \right)\\
% \aleq & \eta^t (x_t^\top \Omega^{-1} x_t) +  \eta^{t+1}\psi + \psi \sum_{i=1}^T \eta^{i} - \psi\sum_{i=1}^{t+1} \eta^{i}\\
% = & \eta^t (x_t^\top \Omega^{-1} x_t) + \psi \sum_{i=1}^T \eta^{i} - \psi\sum_{i=1}^{t} \eta^{i}\\
% \beq & \eta^t (x_t^\top \Omega^{-1} x_t) + \psi \eta \frac{\eta^T - \eta^t}{\eta - 1},
% \end{aligned}
% $$
% where $(a)$ follows since $\eta < \frac{1}{1-\beta}$ and $(b)$ from the relationship $\eta \frac{\eta^T - \eta^t}{\eta - 1} = \sum_{i=1}^T \eta^{i-1} - \sum_{i=1}^t \eta^{i}$. As a consequence, by definition we have $\mathbb{E}[\zeta_{t+1}|\zeta_t] \leq \zeta_t$, hence $\zeta_t$ is a supermartingale. The non-negative follows easily by observing that $\eta > 1, \psi \geq  0 $ by assumption, and $x_t^\top \Omega^{-1}x_t \geq 0$ for all $x_t \in \mathbb{R}^n$ since $\Omega^{-1} \succ 0$.  
% \end{proof}

Next, we show how the nonnegative supermartingale defined in Lemma \eqref{lemma:super} can be used together with Lemma \eqref{lemma:Ville} to ensure the sought probabilistic guarantees.

\begin{proposition}\label{prop:Ville}
Let \eqref{eq:safety:martingale} hold for all $t  = 0,\ldots, T$ and define $\mathcal{B} = \{ x \in \mathbb{R}^n \; : \; 1 - x^\top \Omega^{-1}x \geq 0\}$. Pick $\beta \in (0,1) \delta \geq 0, \eta \in (1, \frac{1}{1-\beta}]$ and define $\psi = \beta + \delta$. Then
$$
\mathbb{P}(x_t \in \mathcal{B}, \forall t = \{0,\ldots,T\}) \geq 1 - \alpha,
$$
with $\alpha = \frac{1-b(x_0)+ \psi \eta \frac{\eta^T - 1}{\eta - 1}}{\eta^T}.$
\end{proposition}

% \begin{proof} 
% We shall exploit $\zeta_t$ constructed in Lemma \eqref{lemma:super}. By Lemma \eqref{lemma:Ville}), for any given $a > 0$ it holds
% \begin{equation}\label{eq:fin:1}
% \text{Pr}\left(\sup_{0 \leq t \leq T} \zeta_t > a \right) \leq \mathbb{E}[\zeta_0]/a.
% \end{equation}
% Recall the safety description in \eqref{eq:safety:finite:recap}. Our goal is to then find an $a^\star$ such that 
% \begin{equation}\label{eq:fin:1a}
% \left(\sup_{0 \leq t \leq T} \zeta_t \leq  a^\star \right) \implies \left( \inf_{0 \leq t \leq T} b(x_t) \geq -\gamma \right),
% \end{equation}
% where $\gamma > 0$ describes the super-level set representing the safe set. In our case, we fix $\gamma = 0$ (and hence drop it consequently); however, one can use the same argument to analyze any super-level set of interest.  Note that by \eqref{eq:fin:1} and \eqref{eq:fin:1a}, we can bound the safety probability as
% \begin{equation}\label{eq:fin:2}
% \begin{aligned}
% & \text{Pr}(x_t \in \mathcal{B}, \forall t = \{0,\ldots,T\}) \\
% = & \text{Pr}\left( \inf_{0 \leq t \leq T} b(x_t) \geq 0 \right) \\
% = &  \text{Pr}\left(\sup_{0 \leq t \leq T} \zeta_t \leq a^\star \right) \\
% = &  1 - \text{Pr}\left(\sup_{0 \leq t \leq T} \zeta_t > a^\star \right)\\
% \geq & 1 - \mathbb{E}[\zeta_0]/a^\star.
% \end{aligned}
% \end{equation}

% Consider 
% \begin{equation}\label{eq:a:def}
% a_t = \eta^t + \frac{\psi \eta}{\eta - 1}(\eta^T - \eta^t)
% \end{equation}
% and define $a^\star = \min_{t \in \{0,\ldots, T\}} a_t$. Since in \eqref{eq:fin:1a} we assume $\sup_{0 \leq t \leq T} \zeta_t  \leq a^\star$ holds, we have
% $$
% \begin{aligned}
% 0 \geq & \zeta_t - a^\star \ageq  \zeta_t - a_t \\
% = & \left( \eta^t (x_t^\top \Omega^{-1} x_t) + \psi \eta \frac{\eta^T - \eta^t}{\eta - 1} \right) - \left( \eta^t + \frac{\psi \eta}{\eta - 1}(\eta^T - \eta^t) \right)\\
% = & \eta^t (x_t^\top \Omega^{-1} x_t - 1)\\
% = & \eta^t \left(-b(x_t)\right).
% \end{aligned}
% $$
% where (a) follows by definition of minimum. Since $\eta > 0$, it holds $b(x_t) \leq 0, \forall t = \{0,\ldots, T\}$ impliying $\inf_{t \in \{0,\ldots,T\}} b(x_t) \geq 0$. Next, consider \eqref{eq:a:def} and notice that $a^\star$ is obtained for $t = T$ for $\eta \in (1, \frac{1}{1-\beta})$. In fact, $a_t = \eta^t \underbrace{\left[1 - \frac{\psi \eta}{\eta - 1} \right]}_{\kappa} + \frac{\psi \eta}{\eta - 1}\eta^T$ with $\kappa < 0$ in the specified interval of $\eta$; hence, $a_t$ is a decreasing function in $t$. By \eqref{eq:fin:1} we then get
% $$
% \begin{aligned}
%  \text{Pr}(\sup_{0 \leq t \leq T} \zeta_t > a^\star) 
% & \leq   \frac{x_0^\top \Omega^{-1} x_0 + \psi \eta \frac{\eta^T - 1}{\eta - 1}}{ \eta^T}\\
% & = \frac{1-b(x_0)+ \psi \eta \frac{\eta^T - 1}{\eta - 1}}{\eta^T}.
% \end{aligned}
% $$
% and as consequence
% $$
%  \text{Pr}(x_t \in \mathcal{B}, \: \forall t \in \{0,\ldots, T\}) \geq 1 - \frac{1-b(x_0)+ \psi \eta \frac{\eta^T - 1}{\eta - 1}}{\eta^T}.
% $$
% Setting $\alpha = \frac{1-b(x_0)+ \psi \eta \frac{\eta^T - 1}{\eta - 1}}{\eta^T}$ conclude the proof.
% \end{proof}

Before proceeding, we briefly comment on the bound obtained in Proposition \eqref{prop:Ville}. The probability of safety increases the more the initial condition is further away from the safe set border (e.g., higher $b(x_0)$). Further, notice that $\eta \in (1, \frac{1}{\beta}]$ is a free design parameter that can be selected to maximize the safety probability. By \cite[Lemma~2]{cosner2023robust}, the function 
$$
\alpha(\eta) =  \frac{1-b(x_0)+ \psi \eta \frac{\eta^T - 1}{\eta - 1}}{\eta^T} 
$$
has first-order derivative
$$
\frac{d \alpha(\eta)}{d \eta}  = -\frac{1-b\left(\mathbf{x}_0\right)} T \eta^{-T-1}-\psi\sum_{t=1}^T{(T-t) \eta^{t-T-1}} \leq 0,
$$
hence it is a monotonically decreasing function in the interval $\eta \in (1, \frac{1}{1-\beta}]$. Therefore, we select $\eta^\star = \frac{1}{1-\beta}$ and correspondingly obtain the tightest achievable bound
\begin{equation}\label{eq:tight:bound}
\begin{aligned}
 & \text{Pr}(x_t \in \mathcal{B}, \: \forall t \in \{0,\ldots, T\}) \\
 \geq & 1- \frac{1-b(x_0) + \frac{\beta + \delta}{\beta}((1-\beta)^{-T} - 1)}{(1-\beta)^{-T}}.
 \end{aligned}
\end{equation}
Consequently, for a given risk tolerance $\alpha \in (0,1)$, task horizon $T$ and coefficient $\beta \in (0,1)$, one can select $\delta \geq 0$ and the set of initial condition $\mathcal{I}$ to ensure $\frac{1-b(x_0) + \frac{\beta + \delta}{\beta}((1-\beta)^{-T} - 1)}{(1-\beta)^{-T}} \leq \alpha$. Notice that the above relationship is linear in the decision variable $\delta$, hence, it can be easily enforced in an optimization problem. Armed with these insights, we are now ready to formalize a convex program guaranteeing finite-horizon safety as per Definition \ref{def:finite:safety} with a user-defined tolerance $\alpha$.

Fix $\alpha, \beta \in (0,1)$ and let $\tilde{\beta} = 1 - \beta$. In line with Assumption \ref{ass:sets}, consider an ellipsoidal initial set $\mathcal{I} = \{x \in \mathbb{R}^n \; : \; 1 - x^\top R x \geq \mu\}$, where $R = R^\top \succ 0$ while $\mu$ is to be designed. Further, consider the following \textit{jointly convex} optimization problem:
\begin{subequations}\label{eq:convex-without-input-constraints-finite}
\begin{align}
    \max~&\mathrm{Tr}(\Omega)\\
    \mathrm{subject~to}~& \mu \in (0,1), \delta \in (0,1),\\
    &0\prec\Omega=\Omega^\top\in\mathbb{R}^n, Y\in\mathbb{R}^{m\times n} \label{eq:convex-fin-b}\\
    &\begin{bmatrix}
        \lambda I& \Sigma^{1/2}\\
        \star&\Omega
    \end{bmatrix}\succeq 0,\label{eq:convex-fin-n}\\ 
    & \beta + \delta - \lambda \geq 0,\label{eq:convex-fin-m}\\
    &\begin{bmatrix}
        \tilde{\beta}\Omega&\Omega A^\top +B^\top Y^\top \\
        \star&\Omega
    \end{bmatrix}\succeq 0,\label{eq:convex-fin-e}\\
     &\begin{bmatrix}
     R&I\\I&\Omega
     \end{bmatrix}\succeq 0,\label{eq:convex-fin-f}\\
    & 1 + \theta_1 \delta + \theta_2 \mu \leq \alpha,\\
    &1-a_j^\top \Omega a_j\ge 0,j=1,\ldots,q,\label{eq:convex-fin-h}
\end{align}
\end{subequations}
where $\Omega$ and $Y$ are decision variables, while $\theta_1 = \frac{(1-\beta)^{-T} - 1}{\beta(1-\beta)^{-T}}, \theta_2 = \frac{1}{(1-\beta)^{-T}}$ are known constant. The following theorem constitutes the main result of this subsection. %We show next that \eqref{eq:convex-without-input-constraints} provides a convex design procedure for the synthesis of a valid CBF and feedback controller for \eqref{eq:poly:sys}, certifying infinite-horizon safety according to Definition \eqref{def:bounded:safety}. 

\begin{tcolorbox}[colback=purple!6, colframe=white, sharp corners=south, boxrule=0pt,boxsep=-0.5mm]
\begin{theorem}\label{th:convex-design}
    Consider system \eqref{eq:poly:sys}, safe set $\mathcal{S}$, and initial set $\mathcal{I}$. Let Assumptions \eqref{ass:noise} and consider $\mathbb{W} = \mathbb{R}^n$ and $\mathcal{U}=\mathbb{R}^m$. Further, fix $\alpha \in (0,1)$. Assume that a solution to \eqref{eq:convex-without-input-constraints-finite} exists and is denoted by $\Omega,R,Y,\{\sigma_j\}_{j=1}^q$. Set $u = u(x)=Y\Omega^{-1}x$. Then system \eqref{eq:poly:sys} under $u(x)$ is $\alpha$-safe according to Definition \eqref{def:finite:safety}.
\end{theorem}
\end{tcolorbox}



% We are now ready to prove the main result of the subsection.

% \begin{proof}

% We first prove that \eqref{eq:convex-fin-n}, \eqref{eq:convex-fin-m} and \eqref{eq:convex-fin-e} provide a convex reformulation for \eqref{eq:safety:martingale}. By Assumption \eqref{ass:noise}, condition \eqref{eq:safety:martingale} under the parametrization in \eqref{eq:parametrization:all} evaluates as
% $$
% \begin{aligned}
% &1 - (Ax + BY\Omega^{-1}x)^\top \Omega^{-1}(Ax + BY\Omega^{-1}x) \\
% & - \tilde{\beta}(1 - x^\top \Omega^{-1}x)- \delta - \text{Tr}(\Omega^{-1} \Sigma) \geq 0
% \end{aligned}
% $$
% where $\tilde{\beta} = 1 - \beta \in (0,1)$. This can equivalently be written as
% $$
% \begin{cases}
%  x^\top (\tilde{\beta} \Omega^{-1} - (A + BY\Omega^{-1})^\top \Omega^{-1}(A+BY\Omega^{-1})) x \succeq 0\\
%  \beta - \delta - \text{Tr}(\Omega^{-1}\Sigma) \geq 0.
% \end{cases}
% $$
% We focus on the first condition. From \eqref{eq:convex-fin-b}, we directly have $\Omega$ is invertible. Pre- and post-multiplying the matrix by $\mathrm{diag}(\Omega,I)$, we get
%     \begin{align*}
%         &\begin{bmatrix}
%             \tilde{\beta}\Omega^{-1}&A^\top \Omega^{-1}+\Omega^{-1}B^\top Y^\top \Omega^{-1}\\
%             \star&\Omega^{-1}
%         \end{bmatrix}\succeq 0,\forall x\in\mathbb{R}^n\\
%         &\begin{bmatrix}
%             \tilde{\beta}\Omega^{-1}&(A+BY\Omega^{-1})^\top \Omega^{-1}\\
%             \star&\Omega^{-1}
%         \end{bmatrix}\succeq 0,\forall x\in\mathbb{R}^n.
%     \end{align*}
%     Applying a congruent transformation $\mathrm{diag}(I_n,\Omega)$, we get
%     \begin{equation*}
%         \begin{bmatrix}
%             \tilde{\beta}\Omega^{-1}&(A+BY\Omega^{-1})^\top \Omega^{-1}\\
%             \star&\Omega
%         \end{bmatrix}\succeq 0,\forall x\in\mathbb{R}^n.
%     \end{equation*}
%     Given that $\beta>0$ and $\Omega\succ 0$, we can apply Schur complement to obtain an equivalent condition:
%     \begin{equation}
%         \tilde{\beta}\Omega^{-1}-\star \Omega^{-1}(A+BY\Omega^{-1})\succeq 0,\forall x\in\mathbb{R}^n.
%     \end{equation}
%     By multiplying vector $x$ on both sides of the matrix, we conclude the first case. Next, we focus on the second. By Schur complement it equals to
%     $$
%     \beta - \delta - \lambda \geq 0, \: \begin{bmatrix}\lambda I & \Sigma^{1/2} \\ \star & \Omega \end{bmatrix} \succeq 0
%     $$



% Next we consider the condition $1 - x^\top \Omega^{-1} x \geq \mu$ for all $x \in \mathcal{I} \subseteq \mathcal{B}$. We encode the first inclusion as
% $$
% \{ x \in \mathbb{R}^n | (1-\mu) - x^\top R x\} \subseteq \{ x \in \mathbb{R}^n | 1 - x^\top \Omega^{-1} x\},
% $$
% which is trivially satisfied if $\mu \in (0,1)$ and \eqref{eq:convex-fin-f} holds. Notice that this prove an upper bound to the RHS of \eqref{eq:tight:bound}. Next, we ensure $\frac{b(x_0)}{(1/(\beta+\delta))^T} \geq \alpha$ for a given $\alpha \in (0,1)$ by enforcing
% $$
% \frac{\mu}{(1/(\beta+\delta))^T} \geq \alpha \iff \mu \geq \alpha (\beta+\delta)^T.
% $$
% Exploiting the expansion $(\beta + \delta)^T = \sum_{k=0}^T \binom{T}{k} \beta^{T-k} \delta^k$, the previous constraint can be encoded via SOS techniques as
% $$
% \mu - \alpha \sum_{k=0}^T \binom{T}{k} \beta^{T-k} \delta^k \in \text{SOS}.
% $$



% Finally, $\mathcal{B} \subseteq \mathcal{S}$ is encoded via \eqref{eq:convex-fin-h} by exploiting Farkas' lemma, as done in Theorem \eqref{th:convex-design}. The proof concludes by invoking Proposition \eqref{prop:Ville} and noticing that $\mathcal{B} \subseteq \mathcal{S}$ implies $\text{Pr}(x_t \in \mathcal{B}, \: \forall t \in \{0,\ldots, T\}) \geq 1 - \alpha.$

% \end{proof}


